Audio-FLAN: An Instruction-Following Dataset for Unified Audio Understanding and Generation of Speech, Music, and Sound

Recent advancements in audio tokenization have significantly enhanced the integration of audio capabilities into large language models (LLMs). However, audio understanding and generation are often treated as distinct tasks, hindering the development of truly unified audio-language models. While instruction tuning has demonstrated remarkable success in improving generalization and zero-shot learning across text and vision, its application to audio remains largely unexplored. A major obstacle is the lack of comprehensive datasets that unify audio understanding and generation. To address this, we introduce Audio-FLAN, a large-scale instruction-tuning dataset covering 80 diverse tasks across speech, music, and sound domains, with over 100 million instances. Audio-FLAN lays the foundation for unified audio-language models that can seamlessly handle both understanding (e.g., transcription, comprehension) and generation (e.g., speech, music, sound) tasks across a wide range of audio domains in a zero-shot manner. The Audio-FLAN dataset is available on HuggingFace and GitHub.

==> tables/dataset_and_length.tex <==
% \begin{table*}{p{2cm}p{3cm}p{2cm}p{2cm}p{5cm}}
\onecolumn
\begin{longtable}{p{2cm}p{6cm}p{6cm}}   % 设置列宽，p{width}表示自动换行
\caption{Detailed information of Datasets}  % 表格标题
\label{tab:dataset2task}  % 表格标签，用于引用
\\  % 用来初始化表格
\hline
\textbf{Domain} &  \textbf{Dataset} &   \textbf{Audio Length (\#hours)} \\
\hline
\endfirsthead  % 每页表头部分
\multicolumn{3}{|c|}{\textit{Continued from the previous page}} \\  % 跨页表头
\hline
\textbf{Domain} &  \textbf{Dataset}  &  \textbf{Audio Length (\#hours)} \\
\hline
\endhead  % 继续表头部分
\hline
\endfoot  % 每页的表尾部分
\hline
\endlastfoot  % 最后一页的表尾部分

% 表格内容
\multirow{22}{*}{Speech} & common voice \cite{ardila2019common}  & $19, 673$  \\  
                         & aidatatang \cite{aidatatang200zh}  & $200$ \\  
                         & libritts-R \cite{koizumi2023librittsr}  & $585$ \\  
                         & libritts \cite{zen2019libritts}  & $586$ \\  
                         & HQ-Conversations \cite{xia2024iscslp}  & $100$ \\  
                         & EmoV\_DB \cite{adigwe2018emotional}  & $9.49$ \\  
                         & VCTK \cite{veaux2017cstr}  & $44$ \\  
                         & MLS \cite{Pratap2020MLSAL}  & $45, 042$ \\  
                         & FLEURS \cite{conneau2023fleurs}  & $17$ \\  
                         & Fluent speech commands \cite{lugosch2019speech}  & $19$ \\  
                         & LibriMix \cite{cosentino2020librimix}  & $500$ \\  
                         & Aishell1 \cite{bu2017aishell}  & $155$ \\  
                         & Aishell2 \cite{du2018aishell}  & $1,036$  \\  
                         & Aishell3 \cite{shi2020aishell}  & $65$  \\  
                         & LJSpeech \cite{ljspeech17}  & $23.9$ \\  
                         & The Parallel Audiobook Corpus \cite{pacorpus18}  & $121$  \\  
                         & HiFi TTS \cite{bakhturina2021hi}  & $291.6$ \\  
                         & KeSpeech \cite{tang2021kespeech}  & $1, 428$ \\  
                         & ESD \cite{zhou2022emotional}  & $29$ \\  
                         & CVSS \cite{jia2022cvss}  & $3, 809$ \\  
                         & ASVSpoof2021 \cite{liu2023asvspoof}  & $1270.5$  \\    
% \hline
    \midrule
    \multirow{19}{*}{Music} & Opencpop \cite{wang2022opencpop}  & $5.2$ \\  % 
                           & m4singer \cite{zhang2022m4singer}  & $29.77$  \\  % 
                           & FreeSound Loop Dataset \cite{ramires2020}  & $34.7$ \\  % 
                           & Opensinger \cite{huang2021multi}  & $50$  \\  % 
                           & MedleyVox \cite{jeon2023medleyvox}  & $1.1$ \\  % 
                           & Vocadito \cite{bittner2021vocadito}  & $0.23$ \\  % 
                           & MoisesDB \cite{pereira2023moisesdb}  & $14.4$ \\  % 
                           & CSD \cite{choi2020children}  & $4.86$ \\  % 
                           & Musiccaps \cite{agostinelli2023musiclm}  & $15.28$\\  %  
                           
                           & GTZAN rhythm \cite{marchand2015gtzan}  & $8.3$ \\  % 
                           & GiantSteps key \cite{knees2015two}  & $20.07$ \\  % 
                           & CCOM-HuQin \cite{zhang2022ccom}  & $4.3$ \\  % 
                           & NSynth \cite{engel2017neural}  & $340$ \\  % 
                           & MedleyDB \cite{bittner2014medleydb}  & $7.45$ \\  % 
                           & Free Music Archive \cite{fma_dataset}  & $8, 232$ \\  % 
                           & AAM \cite{ostermann2023aam}  & $125$ \\  % 
                           & MTG \cite{bogdanov2019mtg}  & $3,777$ \\  % 

    \midrule
    \multirow{11}{*}{Audio}  & Audioset \cite{45857}  & $5208$ \\  % 
                            & VGGSound \cite{chen2020vggsound}  & $550$ \\  % 
                            & Wavcaps \cite{mei2023wavcaps}  & $3, 793.3$\\  % 
                            % & Audioset \cite{45857}  &  Audio Inpainting, Audio Super-resolution \\  % 
                            & freesound \cite{font2013freesound}  & $6446.05$ \\  % 
                            & TAU Urban Acoustic Scenes \cite{heittola2020acoustic}  & $68.18$ \\  % 
                            & Vocal Imitation \cite{kim2018vocal}  & $24$ \\  % 
                            & ESC \cite{piczak2015dataset}  & $2.78$ \\  % 
                            & DNS for VAD \cite{reddy2001interspeech}  & $562.72$ \\  % 
                            & ADD2023 \cite{yi2023add} &   $220$ \\
                            
                            
                            
                            
    \midrule
     \textbf{Total}& \textbf{xx} &  \textbf{xx} \\
    \bottomrule
    
\end{longtable}
% \end{table*}


==> tables/dataset_and_task.tex <==
% \begin{table*}{p{2cm}p{3cm}p{2cm}p{2cm}p{5cm}}
\onecolumn
\begin{longtable}{p{2cm}p{6cm}p{6cm}}   % 设置列宽，p{width}表示自动换行
\caption{Detailed information of Datasets}  % 表格标题
\label{tab:dataset2task}  % 表格标签，用于引用
\\  % 用来初始化表格
\hline
\textbf{Domain} &  \textbf{Dataset} &   \textbf{Task} \\
\hline
\endfirsthead  % 每页表头部分
\multicolumn{3}{|c|}{\textit{Continued from the previous page}} \\  % 跨页表头
\hline
\textbf{Domain} &  \textbf{Dataset}  &  \textbf{Task} \\
\hline
\endhead  % 继续表头部分
\hline
\endfoot  % 每页的表尾部分
\hline
\endlastfoot  % 最后一页的表尾部分

% 表格内容
\multirow{22}{*}{Speech} & common voice \cite{ardila2019common}  & TTS, ASR, Language Identification,  \\  
                         & aidatatang \cite{aidatatang200zh}  & TTS,  ASR, Language Identification, \\  
                         & libritts-R \cite{koizumi2023librittsr}  & TTS, SNR Estimation, Descriptive TTS, Zero-shot TTS,  ASR, Language Identification, Gender Recognition, Speaker Verification, Speech Caption, Phonetic Recognition, Spoken Paragraph Recognition \\  
                         & libritts \cite{zen2019libritts}  & TTS, SNR Estimation, Descriptive TTS, Zero-shot TTS \\  
                         & HQ-Conversations \cite{xia2024iscslp}  & TTS, ASR, Accent Recognition, Age Recognition, device Recognition, Gender Recognition, Language Identification, Speaker Verification \\  
                         & EmoV\_DB \cite{adigwe2018emotional}  & TTS, ASR, SV, Language Identification \\  
                         & VCTK \cite{veaux2017cstr}  & TTS, ASR \\  
                         & MLS \cite{Pratap2020MLSAL}  & TTS, ASR, Language Identification \\  
                         & FLEURS \cite{conneau2023fleurs}  & TTS, ASR, Speech-to-Speech translation, Speech-to-text translation, Language Identification \\  
                         & Fluent speech commands \cite{lugosch2019speech}  & TTS, zero-shot TTS, ASR, SV, Gender Recognition \\  
                         & LibriMix \cite{cosentino2020librimix}  & TSE \\  
                         & Aishell1 \cite{bu2017aishell}  & TTS, Gender Recognition, Language Recognition, SV, ASR \\  
                         & Aishell2 \cite{du2018aishell}  & TTS, Gender Recognition, Language Recognition, SV, ASR  \\  
                         & Aishell3 \cite{shi2020aishell}  & TTS,  Gender Recognition, Language Recognition, SV, ASR, Phonetic Recognition  \\  
                         & LJSpeech \cite{ljspeech17}  & TTS, ASR, Language Recognition \\  
                         & The Parallel Audiobook Corpus \cite{pacorpus18}  & TTS, Gender Recognition, Language Recognition, SV, ASR  \\  
                         & HiFi TTS \cite{bakhturina2021hi}  & TTS, ASR, SV, Language Identification \\  
                         & KeSpeech \cite{tang2021kespeech}  & TTS, ASR, SV, Gender Recognition, Age Recognition, Dialect Identification \\  
                         & ESD \cite{zhou2022emotional}  & TTS, Emotional TTS, Voice Conversion, Zero-shot Emotional TTS, Emotion Recognition, Language Identification, SV, ASR \\  
                         & CVSS \cite{jia2022cvss}  & TTS, Speech-to-Text Translation \\  
                         & ASVSpoof2021 \cite{liu2023asvspoof}  & TTS, Deepfake Detection,  \\  
                         & DNS \cite{reddy2001interspeech}  & Denosing, Dereverberation, Declipping, Bandwidth Extension,   \\  
% \hline
    \midrule
    \multirow{19}{*}{Music} & Opencpop \cite{wang2022opencpop}  & Lyrics2song Generation, Singing Voice Synthesis \\  % 
                           & m4singer \cite{zhang2022m4singer}  & Singing Voice Conversion  \\  % 
                           & FreeSound Loop Dataset \cite{ramires2020}  & Text-to-music Generation \\  % 
                           & Opensinger \cite{huang2021multi}  & Singing Voice Conversion, Lyrics2song Generation, Singing Voice Synthesis  \\  % 
                           & MedleyVox \cite{jeon2023medleyvox}  & Text-guided Source Separation \\  % 
                           & Vocadito \cite{bittner2021vocadito}  & Lyrics2song Generation, Singing Voice Synthesis \\  % 
                           & Moises \cite{pereira2023moisesdb}  & Text-guided Source Separation \\  % 
                           & CSD \cite{choi2020children}  & Singing Voice Synthesis, Lyrics2song Generation \\  % 
                           & Musiccaps \cite{agostinelli2023musiclm}  & Music Caption, Text-to-music Generation\\  %  
                           
                           & GTZAN rhythm \cite{marchand2015gtzan}  & Tempo Comparison \\  % 
                           & GiantSteps key \cite{knees2015two}  & Key Comparison \\  % 
                           & CCOM-HuQin \cite{zhang2022ccom}  & Instrumental Technique Classification, Instrumental Technique Comparison \\  % 
                           & vocadito \cite{bittner2021vocadito}  & Beat-level Pitch Estimation, \\  % 
                           & NSynth \cite{engel2017neural}  & Instrument Classification, Pitch Classification \\  % 
                           & MedleyDB \cite{bittner2014medleydb}  & Melody Extraction \\  % 
                           & Free Music Archive \cite{fma_dataset}  & Artist Identification \\  % 
                           & AAM \cite{ostermann2023aam}  & Instrument Classification, Key Detection, Beat Tracking, Chord Estimation, Beat-level Instrument Recognition, Beat-level Pitch Estimation \\  % 
                           & CSD \cite{choi2020children}  & Genre Classification, Beat-level Pitch Estimation \\  % 
                           & MTG \cite{bogdanov2019mtg}  & Emotion Classification, Instrument Classification, Genre Classification, Music Tagging \\  % 

    \midrule
    \multirow{11}{*}{Audio}  & Audioset \cite{45857}  & Text-guided Audio Generation, Time-grounded Text-to-audio Generation, Text-to-audio Retrieval, Audio Captioning, Speech, Silence, Music and Noise Classification, Sound Event Detection, Sound Event Sequence Recognition \\  % 
                            & VGG \cite{chen2020vggsound}  & Label-querying Sound Extraction, Audio-querying Sound Extraction \\  % 
                            & Wavcaps \cite{mei2023wavcaps}  & Text-guided Audio Source Separation, Audio Continuation\\  % 
                            % & Audioset \cite{45857}  &  Audio Inpainting, Audio Super-resolution \\  % 
                            & freesound \cite{font2013freesound}  & Text-guided Audio Generation, Audio Captioning \\  % 
                            & TAU Urban Acoustic Scenes \cite{heittola2020acoustic}  & Acoustic Scene Classification\\  % 
                            & Vocal Imitation \cite{kim2018vocal}  & Audio Understanding \\  % 
                            & ESC \cite{piczak2015dataset}  & Audio-to-audio Retrieval, \\  % 
                            & DNS for VAD \cite{reddy2001interspeech}  & Voice Activity Detection \\  % 
                            & Speech NonSpeech Detection \cite{mei2023wavcaps}  & Speech Nonspeech Detection \\  % 
                            & ADD2023 \cite{yi2023add} &   Deepfake Audio Detection, Voice Activity Detection \\
                            
                            
                            
                            
    \midrule
     \textbf{Total}& \textbf{xx} &  \textbf{xx} \\
    \bottomrule
    
\end{longtable}
% \end{table*}


==> tables/qwen2-tuning-results-all.tex <==

\onecolumn
% \usepackage{array}
\begin{longtable}[hbtp]{p{4.6cm}<{\raggedright}p{4.5cm}<{\raggedright}p{4.5cm}<{\raggedright}}   % 设置列宽，p{width}表示自动换行
\caption{Evaluation results of Qwen2 tuning results. \lmxue{select some tasks in main paper, and move all tasks to appendix. } }  % 表格标题
\label{tab:qwen2_tuning_result}  % 表格标签，用于引用
\\  % 用来初始化表格
\hline
\textbf{Tasks} & \textbf{Results after tuning} & \textbf{Results w/o tuning}\\
\hline
\endfirsthead  % 每页表头部分
\multicolumn{3}{|c|}{\textit{Continued from the previous page}} \\  % 跨页表头
\hline
\textbf{Tasks} & \textbf{Results after tuning} & \textbf{Results w/o tuning}\\
\hline
\endhead  % 继续表头部分
\hline
\endfoot  % 每页的表尾部分
\hline
\endlastfoot  % 最后一页的表尾部分

% \toprule
    % Tasks & Results after tuning & Results w/o tuning  \\  % 表头
    % \midrule % Speech Tasks
    Age Recognition & \textit{MAE}=3.7092, \textit{MSE}=22.9723 & \textit{MAE}=5.3288, \textit{MSE}=47.1621 \\  % 行数据
    Speech-to-text Translation & \textit{WER}=1.0768, \textit{BLEU-1}=0.2746, \textit{BLEU-4}=0.0928, \textit{METEOR}=0.3055, ROUGE\_L=0.2198, \textit{CIDEr}=0.8853 & \textit{WER}=4.5813, \textit{BLEU-1}=0.0594, \textit{BLEU-4}=0.0097, \textit{METEOR}=0.1645, \textit{ROUGE\_L}=0.0668, \textit{CIDEr}=0.1171\\
    Speech Caption & \textit{BLEU-1}=0.6508, \textit{BLEU-4}=0.3970, \textit{METEOR}=0.3908, \textit{ROUGE\_L}=0.5717, \textit{CIDEr}=0.8700 & \textit{BLEU-1}=0.0830, \textit{BLEU-4}=0.0020, \textit{METEOR}=0.0973, \textit{ROUGE\_L}=0.0627, \textit{CIDEr}=0.0077\\
    Automatic Speech Recognition & \textit{WER}=0.7021 & \textit{WER}=1.1941 \\
    Gender Recognition & \textit{ACC}=0.9834 & \textit{ACC}=0.8773\\
    Dialect Identification & \textit{ACC}=0.7264 & \textit{ACC}=0.6644\\
    Emotion Recognition (speech) & \textit{ACC}=0.8260 & \textit{ACC}=0.3801\\
    Language Identification & \textit{ACC}=0.6270 & \textit{ACC}=0.3916\\
    Vocoder Type Classification & \textit{ACC}=0.5447	& \textit{ACC}=0.1835\\
    Spoken Paragraph Recognition & \textit{EER}=0.4628 & \textit{EER}=0.5093 \\
    Speaker Verification & \textit{EER}=0.4614 & \textit{EER}=0.5030 \\
    Phonetic Recognition & \textit{WER}=0.1949 & /\\
    Speaker Identification & / & / \\
    \midrule
    Music Genre Recognition & \textit{ACC}=0.2432 & \textit{ACC}=0.0911\\
    Music Genre Recognition & \textit{ACC}=0.1745 & \textit{ACC}=0.0055\\ % (Multiple) 
    Emotion Recognition (music) & \textit{ACC}=0.1756 & \textit{ACC}=0.0683\\
    Artist Identification & \textit{ACC}=0.3681 & /\\
    
    Instrument Classification & \textit{ACC}=0.5723 & / \\ % (Single) 
    Instrumental Technique Recognition & \textit{ACC}=0.8857 & \textit{ACC}=0.2507\\
    
    Music Tagging & ? & \textit{BLEU-1}=0.0117, \textit{BLEU-4}=0.0034, \textit{METEOR}=0.0932, \textit{ROUGE\_L}=0.0216, \textit{CIDEr}=0.0089 \\ % 核对一下tuning的结果
    Beat Tracking & \textit{ACC}=0.9138 & / \\
    Key Detection & ACC=0.3601 & ACC=0.1272 \\
    Chord Estimation & \textit{ACC}=0.5015 & \textit{ACC}=0.4464\\
    Chord Estimation (time-step) & \textit{OLP}=0.4002 & / \\
    Pitch Classification & \textit{ACC}=0.8196 & \textit{ACC}=0.4725 \\ % (Single) 
    Instrument Recognition & \textit{ACC}=0.797 & \textit{ACC}=0.6107\\ % (CHOICE)
    Instrument Recognition & \textit{ACC}=0.3963 & \textit{ACC}=0.2507\\ % (Multiple) 
    
    Beat-level Pitch Estimation & \textit{ACC}=0.2131 & /\\
    Beat-level Instrument Recognition & \textit{ACC}=0.5384 & /\\
       
    Key Comparison & \textit{ACC}=0.9113 & \textit{ACC}=0.1417 \\
    Tempo Comparison & \textit{ACC}=0.4563 & \textit{ACC}=0.4052 \\
    Instrument Comparison & \textit{ACC}=0.8597	& \textit{ACC}=0.056 \\
    Instrumental Technique Comparison & \textit{ACC}=0.9408	& \textit{ACC}=0.1505\\
    
    Music Caption (CHOICE) & \textit{ACC}=0.6952 & \textit{ACC}=0.3115\\
    Music Caption & \textit{BLEU-1}=0.4295, \textit{BLEU-4}=0.2612, \textit{METEOR}=0.2347, \textit{ROUGE\_L}=0.4384, \textit{CIDEr}=1.4679 & \textit{BLEU-1}=0.1036, \textit{BLEU-4}=0.0249, \textit{METEOR}=0.0774, \textit{ROUGE\_L}=0.1147, \textit{CIDEr}=0.1165\\
    Pitch Change Detection & / & / \\

    \midrule
    Acoustic Scene Classification & \textit{ACC}=0.3666 & \textit{ACC}=0.0634\\
    Sound Event Sequence Recognition & %\textit{ACC}=0.3733, 
\textit{BLEU-1}=0.3323, \textit{BLEU-4}=0.3555, \textit{METEOR}=0.2401, \textit{ROUGE\_L}=0.4062, \textit{CIDEr}=1.7834 & %\textit{ACC}=/,
\textit{BLEU-1}=0.0162, \textit{BLEU-4}=0.0030, \textit{METEOR}=0.0854, \textit{ROUGE\_L}=0.0596, \textit{CIDEr}=0.0692 \\
    Speech, Silence, Music and Noise Classification & \textit{ACC}=0.9757 &	\textit{ACC}=0.6721\\
    Audio Captioning & \textit{BLEU-1}=0.1285, \textit{BLEU-4}=0.0369, \textit{METEOR}=0.1951, \textit{ROUGE\_L}=0.2886, \textit{CIDEr}=0.9735 & \textit{BLEU-1}=0.0150, \textit{BLEU-4}=0.0027, \textit{METEOR}=0.0904, \textit{ROUGE\_L}=0.0439, \textit{CIDEr}=0.0203\\
    Audio Understanding & \textit{BLEU-1}=0.6971, \textit{BLEU-4}=0.6522, \textit{METEOR}=0.4610, \textit{ROUGE\_L}=0.7461, \textit{CIDEr}=0.0621 & \textit{BLEU-1}=0.1614, \textit{BLEU-4}=0.0225, \textit{METEOR}=0.1497, \textit{ROUGE\_L}=0.1433, \textit{CIDEr}=0.0185 \\
    Sound Event Detection & \textit{TOR}=0.4197 & \textit{TOR}=0.0341\\
    Sound Event Detection & ACC=1.0000 & ACC=0.8310 \\ % (3_AudioSet这个任务的所有答案都是yes，需要修改)
    \bottomrule

\end{longtable}
\twocolumn


% tasks not shown in the table
% Intent Classification

==> tables/qwen2-tuning-results-main.tex <==

\onecolumn
% \usepackage{array}
\begin{longtable}[hbtp]{p{4.6cm}<{\raggedright}p{4.5cm}<{\raggedright}p{4.5cm}<{\raggedright}}   % 设置列宽，p{width}表示自动换行
\caption{Evaluation results of Qwen2 tuning results. \lmxue{select some tasks in main paper, and move all tasks to appendix. } }  % 表格标题
\label{tab:qwen2_tuning_result}  % 表格标签，用于引用
\\  % 用来初始化表格
\hline
\textbf{Tasks} & \textbf{Results after tuning} & \textbf{Results w/o tuning}\\
\hline
\endfirsthead  % 每页表头部分
\multicolumn{3}{|c|}{\textit{Continued from the previous page}} \\  % 跨页表头
\hline
\textbf{Tasks} & \textbf{Results after tuning} & \textbf{Results w/o tuning}\\
\hline
\endhead  % 继续表头部分
\hline
\endfoot  % 每页的表尾部分
\hline
\endlastfoot  % 最后一页的表尾部分

% \toprule
    % Tasks & Results after tuning & Results w/o tuning  \\  % 表头
    % \midrule % Speech Tasks
    Age Recognition & \textit{MAE}=3.7092, \textit{MSE}=22.9723 & \textit{MAE}=5.3288, \textit{MSE}=47.1621 \\  % 行数据
    Speech-to-text Translation & \textit{WER}=1.0768, \textit{BLEU-1}=0.2746, \textit{BLEU-4}=0.0928, \textit{METEOR}=0.3055, ROUGE\_L=0.2198, \textit{CIDEr}=0.8853 & \textit{WER}=4.5813, \textit{BLEU-1}=0.0594, \textit{BLEU-4}=0.0097, \textit{METEOR}=0.1645, \textit{ROUGE\_L}=0.0668, \textit{CIDEr}=0.1171\\
    Speech Caption & \textit{BLEU-1}=0.6508, \textit{BLEU-4}=0.3970, \textit{METEOR}=0.3908, \textit{ROUGE\_L}=0.5717, \textit{CIDEr}=0.8700 & \textit{BLEU-1}=0.0830, \textit{BLEU-4}=0.0020, \textit{METEOR}=0.0973, \textit{ROUGE\_L}=0.0627, \textit{CIDEr}=0.0077\\
    % Automatic Speech Recognition & \textit{WER}=0.7021 & \textit{WER}=1.1941 \\
    % Gender Recognition & \textit{ACC}=0.9834 & \textit{ACC}=0.8773\\
    % Dialect Identification & \textit{ACC}=0.7264 & \textit{ACC}=0.6644\\
    % Emotion Recognition (speech) & \textit{ACC}=0.8260 & \textit{ACC}=0.3801\\
    Language Identification & \textit{ACC}=0.6270 & \textit{ACC}=0.3916\\
    Deepfake Detection & \textit{ACC}=0.5447	& \textit{ACC}=0.1835\\
    Spoken Paragraph Recognition & \textit{EER}=0.4628 & \textit{EER}=0.5093 \\
    Speaker Verification & \textit{EER}=0.4614 & \textit{EER}=0.5030 \\
    % Phonetic Recognition & \textit{WER}=0.1949 & /\\
    % Speaker Identification & / & / \\
    \midrule
    % Music Genre Recognition & \textit{ACC}=0.2432 & \textit{ACC}=0.0911\\
    % Music Genre Recognition & \textit{ACC}=0.1745 & \textit{ACC}=0.0055\\ % (Multiple) 
    % Emotion Recognition (music) & \textit{ACC}=0.1756 & \textit{ACC}=0.0683\\
    % % Artist Identification & \textit{ACC}=0.3681 & /\\
    
    % Instrument Classification & \textit{ACC}=0.5723 & / \\ % (Single) 
    Instrumental Technique Recognition & \textit{ACC}=0.8857 & \textit{ACC}=0.2507\\
    
    % Music Tagging & ? & \textit{BLEU-1}=0.0117, \textit{BLEU-4}=0.0034, \textit{METEOR}=0.0932, \textit{ROUGE\_L}=0.0216, \textit{CIDEr}=0.0089 \\ % 核对一下tuning的结果
    Beat Tracking & \textit{ACC}=0.9138 & / \\
    % Key Detection & ACC=0.3601 & ACC=0.1272 \\
    % Chord Estimation & \textit{ACC}=0.5015 & \textit{ACC}=0.4464\\
    Chord Estimation (w/ timestep) & \textit{OLP}=0.4002 & / \\
    % Pitch Classification & \textit{ACC}=0.8196 & \textit{ACC}=0.4725 \\ % (Single) 
    % Instrument Recognition & \textit{ACC}=0.797 & \textit{ACC}=0.6107\\ % (CHOICE)
    % Instrument Recognition & \textit{ACC}=0.3963 & \textit{ACC}=0.2507\\ % (Multiple) 
    
    Beat-level Pitch Estimation & \textit{ACC}=0.2131 & /\\
    Beat-level Instrument Recognition & \textit{ACC}=0.5384 & /\\
       
    Key Comparison & \textit{ACC}=0.9113 & \textit{ACC}=0.1417 \\
    Tempo Comparison & \textit{ACC}=0.4563 & \textit{ACC}=0.4052 \\
    Instrument Comparison & \textit{ACC}=0.8597	& \textit{ACC}=0.056 \\
    Instrumental Technique Comparison & \textit{ACC}=0.9408	& \textit{ACC}=0.1505\\
    
    % Music Caption (CHOICE) & \textit{ACC}=0.6952 & \textit{ACC}=0.3115\\
    % Music Caption & \textit{BLEU-1}=0.4295, \textit{BLEU-4}=0.2612, \textit{METEOR}=0.2347, \textit{ROUGE\_L}=0.4384, \textit{CIDEr}=1.4679 & \textit{BLEU-1}=0.1036, \textit{BLEU-4}=0.0249, \textit{METEOR}=0.0774, \textit{ROUGE\_L}=0.1147, \textit{CIDEr}=0.1165\\
    % Pitch Change Detection & / & / \\

    \midrule
    Acoustic Scene Classification & \textit{ACC}=0.3666 & \textit{ACC}=0.0634\\
    Sound Event Sequence Recognition & %\textit{ACC}=0.3733, 
\textit{BLEU-1}=0.3323, \textit{BLEU-4}=0.3555, \textit{METEOR}=0.2401, \textit{ROUGE\_L}=0.4062, \textit{CIDEr}=1.7834 & %\textit{ACC}=/,
\textit{BLEU-1}=0.0162, \textit{BLEU-4}=0.0030, \textit{METEOR}=0.0854, \textit{ROUGE\_L}=0.0596, \textit{CIDEr}=0.0692 \\
    % Speech, Silence, Music and Noise Classification & \textit{ACC}=0.9757 &	\textit{ACC}=0.6721\\
    Audio Captioning & \textit{BLEU-1}=0.1285, \textit{BLEU-4}=0.0369, \textit{METEOR}=0.1951, \textit{ROUGE\_L}=0.2886, \textit{CIDEr}=0.9735 & \textit{BLEU-1}=0.0150, \textit{BLEU-4}=0.0027, \textit{METEOR}=0.0904, \textit{ROUGE\_L}=0.0439, \textit{CIDEr}=0.0203\\
    % Audio Understanding & \textit{BLEU-1}=0.6971, \textit{BLEU-4}=0.6522, \textit{METEOR}=0.4610, \textit{ROUGE\_L}=0.7461, \textit{CIDEr}=0.0621 & \textit{BLEU-1}=0.1614, \textit{BLEU-4}=0.0225, \textit{METEOR}=0.1497, \textit{ROUGE\_L}=0.1433, \textit{CIDEr}=0.0185 \\
    Sound Event Detection & \textit{TOR}=0.4197 & \textit{TOR}=0.0341\\
    % Sound Event Detection & ACC=1.0000 & ACC=0.8310 \\ % (3_AudioSet这个任务的所有答案都是yes，需要修改)
    \bottomrule

\end{longtable}
\twocolumn
